Generative Models of Visually Grounded Imagination

It is easy for people to imagine what a man with pink hair looks like, even if they have never seen such a person before. We call the ability to create images of novel semantic concepts visually grounded imagination. In this paper, we show how we can modify variational auto-encoders to perform this task. Our method uses a novel training objective, and a novel product-of-experts inference network, which can handle partially specified (abstract) concepts in a principled and efficient way. We also propose a set of easy-to-compute evaluation metrics that capture our intuitive notions of what it means to have good visual imagination, namely correctness, coverage, and compositionality (the 3 C's). Finally, we perform a detailed comparison of our method with two existing joint image-attribute VAE methods (the JMVAE method of Suzuki et.al. and the BiVCCA method of Wang et.al.) by applying them to two datasets: the MNIST-with-attributes dataset (which we introduce here), and the CelebA dataset.

==> affine-table.tex <==
\begin{table}
	\centering
	%\scriptsize
	%\tiny
	\caption{
		Comparison of different approaches on
                \mnistaffine test set. Higher numbers are better. Error bars (in
                parentheses) are standard error of the mean.
                For concrete concepts (where all 4 attributes are
                specified),
                we do not use a PoE inference network, and we do not
                report coverage.
                Hyperparameter settings for each result are discussed in the supplementary material.
	}
	\label{tab:metrics}
	\begin{tabular}{cccccc}
		\toprule
		Method & \#Attributes & Coverage (\%) & \Correctness
                (\%) & PoE? & Training set \\
		\midrule
                \telbo & 4 & - & \textbf{90.76 (0.11)} & N & \iid \\
                \jmvae & 4 & - & 86.38 (0.14) & N & \iid \\
                \bivcca  & 4 & - & 80.57 (0.26) & N & \iid \\
                \midrule
		\telbo & 3 & \textbf{90.76 (0.21)} &  77.79 (0.30) & Y
                & \iid \\
		\jmvae & 3 & 89.99 (0.20) & \textbf{79.30 (0.26)} & Y
                & \iid\\
		\bivcca & 3 & 85.60 (0.34) & 75.52 (0.43) & Y & \iid \\
		\midrule
		\telbo & 2 & \textbf{90.58 (0.17)} &  \textbf{80.10
                  (0.47)} & Y & \iid \\
		\jmvae & 2 & 89.55 (0.30) & 77.32 (0.44) & Y & \iid\\
		\bivcca & 2 & 85.75 (0.32) & 75.98 (0.78) & Y & \iid\\
		\midrule	
		\telbo & 1 & \textbf{91.55 (0.05)} & \textbf{81.90
                  (0.48)} & Y & \iid\\
		\jmvae & 1 & 89.50 (0.09) & 81.06 (0.23) & Y & \iid\\
		\bivcca & 1 & 87.77 (0.10) & 76.33 (0.67) & Y & \iid\\
                \midrule
                \telbo & 4 & - & \textbf{83.10 (0.07)} & N & \comp \\
                \jmvae & 4 & - & 79.34 (0.52) & N & \comp \\
                \bivcca & 4 & - & 75.18 (0.51) & N & \comp \\
		\bottomrule
	\end{tabular}
\end{table}


==> intro-old.tex <==
\section{Introduction}


Generative models of images have become increasingly powerful in
recent years, due to progress in autoregressive modeling
(e.g., the pixelCNN model of \citep{pixelCNNpp}),
latent variable modeling
(e.g. the VAE model of \citep{VAE}),
and implicit density modeling
(e.g., the DC-GAN model of \citep{DCGAN}).
In particular, conditional generative models, of the form
$p(\vx|\vy)$, have become quite popular,
since they provide a way to specify the kind of image $\vx$ you want
to generate by changing the input variables $\vy$.

Prior work has considered the case where $\vy$ consists of an
attribute vector (e.g., \citep{Yan2016}),
a sentence
(e.g., \citep{Reed2016generative}),
another image (e.g., \citep{pix2pix}),
etc.
In this paper, we focus on the case where $\vy$ is an attribute
vector, since this allows an easy way to {\em compositionally} specify an
exponential number of images with a small number of bits.
For example, consider the problem of generating images of faces,
with properties specified by 2 binary attributes
is-male and has-beard.
which we will denote by $y_m$, and $y_b$.
We can easily specify $2^2=4$ different ``scenes'' by
``twiddling'' each of these bits.
Some of these combinations (e.g., $(y_m=0,y_b=1)$ corresponding to
females with beards)
might be rare or non-existent in the training data,
but ideally the model should nevertheless be able
to ``imagine'' what such an image
would look like,
so it could generate a ``plausible'' set of samples.\footnote{
  %
We are assuming the training data contains variation
amongst the individual attributes
(e.g., it contains examples with labels $(y_m=1,y_b=1)$
and $(y_m=0,y_b=0)$), but not that
it contains all possible combinations.
}
We can interpret $\vy$ as a way to specify a visual concept.
We say that it is a compositionally novel concept if it has never been seen
before in the training set.

Now suppose that we don't want to generate a specific kind of face,
but rather a whole class of faces, e.g., all male faces.
We can specify this broad visual concept by setting $y_m=1$,
but leaving all the other attributes
unspecified. We call this process {\em visual abstraction}.


We would like all the resulting generated images to contain
male faces, but there should be a mix of images with and without beards.
That is, we want the model to ``cover'' the space of images that
constitutes the ``extension'' of the visual concept ``male face''
by creating a {\em diverse} set of images,
subject to the constraint that all the images match the specified
criteria.
We formalize this notion in \cref{sec:metrics}.

Conditional (discriminative)
generative models of the form $p(\vx|\vy)$ have difficulties
when dealing with missing input data, i.e., when certain components of $\vy$
are unspecfied.
Various heuristics can be used, such as encoding missing attributes
with a special value such as -1,
but this requires that the model learn that such values correspond to
lack of information, which is difficult.
This makes conditional models  hard to use for the visual abstraction
task.
By contrast, joint generative models, of the form $p(\vx,\vy)$, provide a
principled solution to missing data, namely marginalizing out the
missing components. More precisely let $\calO$ be the observed
attributes, and $\calM$ be the missing attributes.
Then we can generate images conditioned only on the observed
attributes by computing
\[
p(\vx|\yobs) = 
\frac{\sum_{\ymiss} p(\vx,\yobs,\ymiss)}
     {\int d \vx' \sum_{\ymiss} p(\vx',\yobs,\ymiss)}
     \]

Computing the various sums and integrals is often intractable.
However, by making certain modeling assumptions, we can get
a much more tractable result.
In particular, let us assume that $\vx$ and $\vy$ are conditionally
independendent given a shared latent factor $\vz$,
so $p(\vx,vy,\vz) = p(\vx|\vz) p(\vy|\vz) p(\vz)$.
Let us also assume that the attributes are conditionally independent,
so $p(\vy|\vz)=\prod_j p(y_j|\vz)$.
Then we can write
\[
p(\vx|\yobs)
= \sum_{\ymiss} p(\vx,\ymiss|\yobs) 
= \sum_{\ymiss} \int d\vz p(\vx|\vz) p(\ymiss|\vz) p(\vz|\yobs) 
= \int d\vz p(\vx|\vz) p(\vz|\yobs) 
\]
since $\sum_{\ymiss} p(\ymiss|\vz)=1$.
Thus we just need to do posterior inference of the latent factors
$\vz$ given the partially observed attribute vector $\yobs$,
and then we can generate images $\vx$ in the usual way.

There are a variety of ways of performing (approximate) posterior
inference in latent variable models,
including MCMC (e.g., \citep{Hoffman2017})
and variational inference (e.g., \citep{Hoffman2013svi}).
Recently it has become popular to use amortized inference,
in which we train an inference network to approximate
the posterior $q(\vz|\vy)$ directly, thus avoiding the need to
perform iterative sampling or iterative optimization.
This approach is used in variational autoencoders (VAEs)
\citep{VAE} and various other models.
However, it has the downside that it cannot handle missing inputs,
as we discussed above.

In \cref{sec:POE}, we discuss a novel solution to this problem,
based on combining VAEs with an inference network
based on a product of experts.
This  enjoys the speed benefits of amortized inference,
with a proper treatment of uncertainy in $\vz$ induced by lack of
information in $\vy$. In particular, we will show that our method
causes $q(\vz|\yobs)$ to have broad support in latent space when
$\yobs$ only specifies a small number of attributes (corresponding to
 a very abstract class), but has narrower support when we specify more
 constraints. This naturally results in our model generating a
set of images whose diversity depends on the level of abstraction of
the concept, as we show experimentally in \cref{sec:experiments}.



==> mnist-table.tex <==
\begin{wraptable}{l}{7cm}
%\begin{table}
  \centering
  	\centering
		\tiny
	
	\label{tab:metrics}
  \begin{tabular}{cccc}
    \toprule

    \textbf{Method}  & \textbf{\#Attributes} & \textbf{Coverage} (\%) & \textbf{\Correctness} (\%)                                \\

    \toprule
    \rowcolor{Gray}\multicolumn{4}{c}{iid split}\\
    \toprule
    % triple ELBO
    \telbo  & \multirow{3}{*}{4} & -            & 82.08 {\tiny$\pm$} 0.56\\
    % JMVAE
    \jmvae  &  & -            & {\bf 85.15} {\tiny$\pm$} 0.26  \\
    % bi-VCCA
    \bivcca &  & -            & 67.38 {\tiny$\pm$} 0.69 \\

    \midrule

    % triple ELBO
    \telbo  & \multirow{3}{*}{3} & {\bf 91.14} {\tiny$\pm$} 0.53 & 81.63 {\tiny$\pm$} 0.38 \\
    % JMVAE
    \jmvae  & & 88.52 {\tiny$\pm$} 0.37 & {\bf 82.00} {\tiny$\pm$} 0.37  \\
    % bi-VCCA
    \bivcca & & 85.28 {\tiny$\pm$} 0.68 & 70.68 {\tiny$\pm$} 0.87  \\

    \midrule

    % triple ELBO
    \telbo  & \multirow{3}{*}{2} & {\bf 90.32} {\tiny$\pm$} 0.57 & {\bf 82.03} {\tiny$\pm$} 1.37  \\
    % JMVAE
    \jmvae  &  & 87.89 {\tiny$\pm$} 0.69 & 81.02 {\tiny$\pm$} 1.05 \\
    % bi-VCCA
    \bivcca &  & 85.09 {\tiny$\pm$} 0.76 & 72.33 {\tiny$\pm$} 2.31 \\

    \midrule

    % triple ELBO
    \telbo  & \multirow{3}{*}{1} & {\bf 90.94} {\tiny$\pm$} 0.19 & {\bf 83.67} {\tiny$\pm$} 1.70 \\
    % JMVAE
    \jmvae  & & 88.70 {\tiny$\pm$} 0.35 & 81.58 {\tiny$\pm$} 1.78 \\
    % bi-VCCA
    \bivcca & & 85.53 {\tiny$\pm$} 0.27 & 68.36 {\tiny$\pm$} 2.21 \\
    
    \toprule
    \rowcolor{Gray}\multicolumn{4}{c}{Compositional split}\\
    \toprule
    % triple ELBO
    \telbo  & \multirow{3}{*}{4} & -            & 75.61 {\tiny$\pm$} 1.43  \\
    % JMVAE
    \jmvae  & & -            & {\bf 76.86} {\tiny$\pm$} 1.30  \\
    % bi-VCCA
    \bivcca & & -            & 68.58 {\tiny$\pm$} 1.02  \\

    \bottomrule
  \end{tabular}
\caption{
	Comparison of different approaches on \MNISTA\
	test set. Higher numbers are better. We report standard deviation
	across 5 splits of the test set.
}
%\end{table}
\end{wraptable}


==> models.tex <==
\section{VAE-based models for visual semantic imagination}
\label{sec:method}
\label{sec:methods}

We start by describing standard VAEs \citep{Kingma2014},
to introduce notation. We then discuss our extensions to handle the
task of visually grounded semantic imagination.

\eat{
We will use $q(z|y)$ to represent the mapping of a concept $y$ to an
internal abstract latent representation $z$.  The concept $y$ is
represented by a (possibly partially specified) attribute vector. We
can ``ground'' this into a set of images, in order to evaluate the 3
C's, by sampling from the distribution $p(x|z)$.  In the following, we
interpret $p(x|z)$ and $q(z|y)$ as generative and inference networks
within VAE-like  models, and discuss how to use
such models to perform imagination tasks.
}

\paragraph{Standard VAEs.}
A VAE \citep{Kingma2014} is a latent variable model of the form
$p_{\theta}(x,z) = p_{\theta}(z) p_{\theta}(x|z)$,
where $p(z)$ is the prior (we assume it is Gaussian,
$p(z)= \gauss(z|0,I)$, although this assumption can be relaxed),
and $p(y|z)$ is the likelihood (sometimes called the decoder), usually represented by a neural network.
To perform approximate posterior inference, we fit an inference
network (sometimes called the encoder) of the form $q_{\phi}(z|x)$,
so as to maximize
maximize 
the evidence lower bound
or ELBO:
\begin{equation}
   \elbo(x) = E_{z \sim q_{\phi}(z | x)}
   [\log p_{\theta}(x | z)] - \KL( q_{\phi}(z| x), p(z) )
\end{equation}
where   $\KL(p,q)$ is the Kullback Leibler divergence between distributions
   $p$ and $q$.
It is easy to show that $\elbo(x) \leq \log p(x)$,
so this is a form of approximate maximum likelihood training.


\paragraph{Joint VAEs and the \telbo.}
\label{sec:elbo}

We extend the VAE to model images and attributes by defining
the joint distribution
$p(x,y,z) = p(z) p(x|z) \prod_{k \in \attributes} p(y_k | z), $
where $p(x|z)$ is the image decoder (we use the DCGAN
architecture from \citep{Radford2016}), and $p(y_k|z)$ is an MLP for
the $k$'th attribute, that maps $z$ to a softmax distribution over the
possible values for $y_k$.
(For more details on the model architectures,
see the supplementary material.)

If we only observe a single modality, we can marginalize out
the non-observed variables.
For example, if we just observe an image, and no attribute,
the conditional likelihood becomes
\begin{equation}
\sum_y p(x,y|z) =  \sum_y \left[ p(x|z) p(y|z) \right]
  = p(x|z) \left[ \sum_y p(y|z) \right] = p(x|z) 
\end{equation}
Similarly, if we just observe a attribute, and no image,
the conditional likelihood becomes $p(y|z)$.

In addition to the generative model,
we fit an inference network of the form $q(z|x,y)$.
To handle the case where we only have an image as input,
we fit a $q(z|x)$ network.
Similarly,
to handle the case where we only have a attributes as input,
we also fit a $q(z|y)$ network.
So overall we fit three inference networks.
The output of each of these networks is two vectors,
one predicting the posterior mean of $z$,
and one predicting its posterior covariance
(we assume the covariance is diagonal for simplicity).


Our objective function for a single datapoint has the following form,
which we call the \emph{\telbo}:
\begin{align}
\label{eqn:triple_elbo}
{\mathcal L}(x,y)
 &=
E_{q(z|x,y)} [\bimodalx \log p(x|z) + \bimodaly \log p(y|z)]
   - \KL(q(z|x,y), p(z)) \nonumber \\
 &  + E_{q(z|x)} [\unimodalx \log p(x|z)] - \KL(q(z|x), p(z))  \nonumber \\
  & + E_{q(z|y)} [\unimodaly \log p(y|z)] - \KL(q(z|y), p(z))
%    = \sum_{(x,y) \in \data_{xy}}
%    \elbo_{\lambda_{x}, \lambda_{y}}(x, y) + \sum_{x \in \data_x} \elbo_{\lambda_x}(x)
%    + \sum_{y \in \data_y} \elbo_{\lambda_y}(y),
\end{align}
where
%    $\data_{x,y} = \{ (\super{x}{n}, \super{y}{n}) \}$ contains images with
%    corresponding attributes, $\data_{x} = \{ \super{x}{n} \}$ contains just
%    images, $\data_{y} = \{ \super{y}{n} \}$ contains just attributes
   $\unimodalx$, $\unimodaly$, $\bimodalx$, $\bimodaly$ are scaling
    terms, chosen to balance the likelihood contribution of each type
    of data.
    (We discuss these terms in more detail later.)
    

%    In Section~\ref{sec:related} we explain
%    how this relates to similar objectives proposed in other papers,
%    and in Section~\ref{sec:results} we show that it works better than
%    these alternatives.

    \paragraph{Justification for the \telbo.}
    We now give an intuitive justification for the \telbo objective.
We want to ensure that the region of latent space
occupied by each attribute vector $y$
matches the region of latent space
occupied by the  set of corresponding $(x,y)$ pairs,
where $x \in \data_{xy}$ is
drawn from the set of images corresponding to $y$.
More precisely,
let $q(z|\data_{xy}) = \frac{1}{|\data_{xy}|} \sum_{x \in \data_{xy}}
q(z|x,y)$
be the ``empirical posterior'' for this grounding of the concept.
We would like $q(z|y)$ to match $q(z|\data_{xy})$,
so it ``covers'' all the examples
of the concept that it has seen.
However, we don't want to only put mass on the observed examples,
or worse a single observed example,
so we also want $q(z|y)$ to be as entropic (\ie, as close
to the $\gauss(0,I)$ prior) as possible.
(The issue of how much to generalize from a small set of examples of a
concept, and along which feature dimensions,
is also discussed in \citep{Tenenbaum99nips}.)

As we explain in Section~\ref{sec:related},
different papers adopt different objectives for encouraging this
    behavior.
In our approach, we rely on the triple ELBO.
This  encourages $q(z|y)$ to be as close as possible
to $q(z|\data_{xy})$,
since the same decoder network $p(y|z)$ is used
for generating both the paired and unpaired data.
Furthermore,
the $\KL(q(z|y), p(z))$ term 
encourages $q(z|y)$ to be as broad as possible,
relative to the length scale defined by the prior.

However, we noticed empirically that sometimes the \telbo on its
own is insufficient to enforce this desired behavior.
To see why, consider generating an attribute vector $y$.
If this attribute vector is paired with an image,
the latent variable will be sampled
from $q(z|x,y)$.
If this is not paired with an image, it will be sampled from $q(z|y)$.
We would like the model to use the same part of latent space in both
cases, so that the representation is shared,
but a powerful decoder could learn to map different parts of latent
space to the same observation.
To avoid this effect,
we only train the parameters of the 
$p(y|z)$ model in the $\elbo(x, y)$ term
and not in the $\elbo(y)$ term.
When optimizing the $\elbo(x,y)$ term on paired data,
the model learns a latent representation based on aligned images and
attributes.
When optimizing the $\elbo(y)$ term, the model just needs to learn how
to map into this precomputed embedding space.
(In practice, we optimize all terms simultaneously,
but conceptually it is helpful to think of a two-step process.)
We call this variant of the model \telbofl,
where FL stands for ``frozen likelihood''.


\eat{
What would be the property of an ideal inference network for
attributes $q(z| y)$? To compute the extension of a concept, one would
expect to span the region in the latent space occupied by the
corresponding images (images of cats) for the concept $y$ (say
cat). Thus, we want $q(z|y)$ to match the aggregate $q(z|x, y)$ across
the space of all images $x$ for the concept $y$. The
$elbo_{\lambda_y}(y)$ implements this as follows. We add a constraint
through this term that irrespective of whether we sample $z_{xy} \sim
q(z| x, y)$ or we sample $z_{y} \sim q(z| y)$, we expect the
likelihood function $p(y|z)$ to produce the correct attribute class as
output. This ensures \correctness, however there is still the danger of
mode collapse (since we could just snap to a particular $q(z| x, y)$
gaussian for an image $x$. Appropriate coverage is then encouraged by
the $KL$-divergence term which requires that $q(z| y)$ have minimal
divergence w.r.t. the prior $p(z)$, while ensuring that we map to a
space where $p(y|z)$ is able to make the correct label assignment.
}



\eat{
Note that in addition to the \telbo, we add some additional
regularization terms. In particular, we use $\ell_1$ regularization
for the weight matrix from $z$ to the first hidden layer of each of
the attribute decoders, $p(y_k|z)$.  This is to encourage each latent
dimension to generate a sparse subset of observed attributes.  For
example, $z_{1:3}$ might encode the bird's color (since it is known
that color can be represented by a 3d space \citep{Bhargava2017}), and
$z_4$ might represent its size.
%and  $\ell_2$ regularization (aka "weight decay") for all the remaining weights. 
%We choose the strength of the regularization parameters based on a validation set.
}

\paragraph{The role of the likelihood scaling terms.}

If the image decoder $p(x|z)$ is a Gaussian,
then we can interpret $\unimodalx \log p(x|z)$
as simply a rescaling of
the precision of this Gaussian,
since
\[
\unimodalx  \log p(x|z) =
-\frac{\unimodalx}{2 \sigma^2} (x-\mu(z))^T \Sigma(z)^{-1}(x-\mu(z))^2
+\mathrm{const}.
\]
where $\mu(z)$ and $\Sigma(z)$ are the outputs of the image decoder
given input $z$. (Typically $\Sigma(z)$ will be diagonal.)

When we have a uni-modality VAE, the scaled objective becomes
\begin{align}
L &= \unimodalx E_{q(z|x)} [\log p(x|z)] - \KL(q(z|x), p(z))\\
 &=  E_{q(z|x)} [\log p(x|z)] - \beta_x \KL(q(z|x), p(z))
\end{align}
where $\beta_x = 1/\unimodalx$.
This is equivalent to the $\beta$-VAE approach
of \citep{Higgins2017}.
They showed that by using $\beta_x \gg 1$, they could encourage the
learning of a ``disentangled'' representation,
since the posterior is forced to be closer to the $\gauss(0,I)$ prior,
which is already disentangled.

When we have a multi-modality VAE, the scaling terms affect not just
how much we regularize towards the prior,
but also how much each modality influences the latent space.
When the modalities have different amounts of information,
it is important to tune these scaling parameters appropriately,
In particular, since an image is more informative than an attribute,
we need to set  $\unimodaly > 1$,
$\unimodalx \leq 1$,
and $\bimodaly / \bimodalx > 1$;
this ensures that the latent space is shared
between the attributes and the images,
as we illustrate in Section~\ref{sec:results2bit}.

\paragraph{Product of Experts (PoE).}
\label{sec:poe}

In order to handle missing attributes at test time, we assume that the
$q(z|y)$ inference network has the following form:
 $ q(z|\concept) \propto p(z) \prod_{k \in \obs} q(z|y_k)$,
where  $q(z|y_k) = \gauss(z
 | \mu_k(y_k), C_k(y_k))$ is the $k$'th Gaussian ``expert'',
and $p(z) = \gauss(z|\mu_0=0, C_0=I)$ is the prior.
This is  similar to the product of experts model
model proposed in \citep{Hinton2002},
but differs in two ways.
First, we include  the ``universal expert'' $p(z)$,
for reasons we discuss in Section~\ref{sec:results2bit}.
Second, we apply this model to represent the distribution of the
latent variables, not the visible variables. 
 
%(This is an example of an
%``exponentially tilted distribution''.)

\eat{
To see why we need the universal expert,
note that when all attributes are present
(as is the case during training),
the only thing that matters is that the product of the Gaussians is
well behaved;
however,
the individual Gaussians can become  very  broad in some
latent dimensions,
as we show in  Figure~\ref{fig:poe}(b).
However,
at test time, some attributes may be missing,
so $q(z|y_{\obs})$ may be a poorly shaped Gaussian.
By always including
$p(z)$ in the product,  we ensure that the resulting
distribution is always reasonably
similar in scale to the prior,
as we show in Figure~\ref{fig:poe}(c).
}

In \citep{Hinton2002}, each expert produced a distribution over binary
variables, similar to a Boltzmann machine, and hence the normalization
constant of the product was intractable. In our case,
it can be shown that the (normalized!) product of all the Gaussian experts
has the form $q(z|\concept) = \gauss(z | \mu, C)$,
where $C^{-1} = \sum_{k} C_k^{-1}$ and
$\mu = C(\sum_k C_k^{-1} \mu_k)$,
where the sum is over all observed attributes plus
the 0 term corresponding to $p(z)$.
This equation has a simple intuitive interpretation:
If we do not observe any attributes, the posterior reduces to the
prior. As we observe more attributes, the posterior becomes narrower,
since the (positive definite) precision matrices add up,
reflecting the increased specificity of the concept being specified,
as we show in Section~\ref{sec:results2bit}.

\eat{
\paragraph{Sparsity promoting prior.}
In the PoE model, we can think of each attribute as acting like a soft constraint on
the latent space distribution.
Ideally, different attributes would correspond to different latent
dimensions, so they can capture orthogonal factors of variation.
 For example,
$z_{1:3}$ might encode a bird's color (since it is known that color
can be represented by a 3d space \citep{Bhargava2017}), and $z_4$
might represent its size.  To encourage this behavior, we use $\ell_1$
regularization for the weight matrix from $z$ to the first hidden
layer of each of the attribute decoders, $p(y_k|z)$.
The benefit of this is illustrated in Figure~\ref{fig:JVAE}(c),
where we show a simple 2d example in which the vertical dimension
represent the parity of a digit, and the horizontal dimension
represents its magnitude.
}


\eat{
\paragraph{Semi-supervised learning.}

Our method can also support semi-supervised learning (SSL), where we
train on images without attributes, $\datassl_{x} = \{
x \sim \ptrue(x) \}$, and/or attributes without images,
$\datassl_{y} = \{ y \sim \ptrue(y) \}$, in addition to paired data,
$\datatrain_{xy}$.  In standard SSL, where the goal is to learn a
classifier, we train on $\datatrain_{xy}$ and $\datassl_{x}$, and test
on $\datatest_{xy}$, If the space of labels $Y$ is richer than classes
(\eg, attributes or natural language captions), we can also train on
$\datassl_{y}$, to better learn any correlations between the
attributes or words.

In the compositional setting, there are several possible options, as
we discuss in more detail in the supplementary material.  We consider
the following scenarios: (1) train on $\datatrain_{xy1}$ and
$\datassl_{y2}$; we call this ``visual imagination'', since the
student is exposed to labels from $\ptwo(x,y) = \ptrue(x,y|y \in
Y_2)$, but not any images.  (2) train on $\datatrain_{xy1}$ and
$\datassl_{x2}$; we call this ``linguistic imagination'', since the
student is exposed to images from $p_2$, but not any attributes.
%
}


\eat{
We focus on two scenarios, one in which we see unlabeled examples from
$\datassl_{x1} = \{ x \sim \ptrue(x|y \in Y_1) \}$ and $\datassl_{x2}
= \{ x \sim \ptrue(x|y \in Y_2) \}$, and a harder case where we just
see unlabeled examples from $\datassl_{x1}$.  In both cases, we also
train on $\datatrain_{xy1}$ and test on $\datatest_{xy}$.  We call the
first case ``semi-supervised compositional generalization''; we call
the second case ``semi-supervised imagination'', since we see
unlabeled images from $Y_1$ (which makes this semi-supervised), but we
do not see any images from $Y_2$ (which makes this an imagination
task).  }






==> results-affine.tex <==
\subsection{\mnistaffine Results}

\subsubsection{Dataset.}

In this section, we use a slightly more complex dataset which we
call ``\mnistaffine'', which stands for ``MNIST with attributes''.
This is created by modifying the original MNIST digits as follows.
We first create  a compositional concept hierarchy using
4 discrete
attributes, corresponding to class label (10 values),
location (4 values),
orientation (3 values), and scale (2 values).
Thus there are \texttt{10x2x3x4=240} unique concepts in total.

Next
we create $\sim 290$ example images of each concept by sampling real-valued
transformation parameters from truncated Gaussian distributions associated with
each attribute value, and then applying the corresponding affine transformation to
randomly chosen MNIST digits  of the corresponding class.\footnote{
  %
  More precisely,
  we generated the dataset as follows:
  for each of the 70k original MNIST images, we sampled 10 attribute
  vectors uniformly at random (keeping the class label consistent with
  the chosen image); we then generated 10 versions of the original
  image, resulting in a dataset of 700k labeled images.
  Thus each concept has about $70,000/240 \approx 291$ images associated
  with it.
  Note that the transformed images are grayscale, just like the original MNIST dataset.
  We binarize the images for training and evaluation.
  See the supplementary material for details.
} %
We call this the \iid dataset.
We split this into a train, validation and test set using
85\%, 5\% and 10\%
of the data, respectively.

We also create a compositional split of the data (denoted \comp),
where we put
85\% of the concepts (204) in the training set,
5\% of the concepts (12) in the validation set,
and 10\% of the concepts (24) in the test set.
The splits are chosen so that each  attribute vector only appears in
one of the three sets.
We convert the training concepts into a dataset of images and
attributes by extracting images with matching attributes from the
\iid dataset.

In addition to the 240 concrete concepts,
we create a set of abstract concepts as follows:
 for each level of abstraction
 (obtained by dropping 1, 2, or 3 of the attributes),
we make 2 variants of each of the 240 possible concepts by
dropping different attributes at random, resulting in 480 abstract
concepts per level.
We repeat the above process of random dropping independently for train,
val and test splits giving us three sets of abstract queries.
(Note that we do not use the abstract training set, since we only
train on concrete concepts; but we do use the abstract validation and
test concepts for evaluating model performance.)

\subsubsection{Evaluation methodology.}

We compare various models  on both the \iid and \comp datasets.
We then evaluate performance in terms of \correctness and coverage
of concrete and abstract concepts.
More precisely, we consider the following scenarios:
(1) train on \iid, evaluate \correctness on previously seen concrete concepts;
(2) train on \iid, evaluate \correctness and coverage on abstract
concepts;
(3) train on \comp, evaluate \correctness on novel concrete concepts.
We do not evaluate coverage of concrete concepts,
since even a single sample will suffice to cover a
concept in which all attributes are specified (providing all the
attributes for the sample match
all the attributes of the concept, \ie, the sample is correct).

To measure correctness and coverage, we need to convert a sampled
image into an attribute vector.
For this,
we train the observation classifier on the full \iid dataset,
where it gets to an accuracy of 91.18\% for
class label, 90.56\% for scale, 92.23\% for orientation, and 100\% for location. 
Consequently, it is a reliable way to assess the quality of samples
from various generative models.


\subsubsection{Models and training.}

For the image models, $p(x|z)$ and $q(z|x)$,
we  use the DCGAN architecture from \citep{Radford2015}).
For the attribute models,  $p(y_k|z)$, $q(z|y_k)$ and $q(z|y_{1:K})$,
we use MLPs.
For the joint inference network, $q(z|x,y)$, we use  a CNN combined with an MLP.
We use $d=10$ latent dimensions for all models.
See supplementary
material for details.

We train each model using three objectives:
\telbo, \jmvae and \bivcca.
We use Adam~\citep{Kingma2015adam} for  
	optimization, with a learning rate of 0.0001, and a minibatch size of 64.
	We train all models for 500,000
	steps (we generally found that the models do not tend to overfit in our
	experiments).
        %In our initial experiments we found the choice of Adam to be
	%cricial to achieve good performance.

\subsubsection{Hyper-parameters.}
        \label{subsec:hyperparams}

For each model,
we have to choose various hyperparameters:
%the number of latent dimensions $d \in \{10, 20\}$,
the label likelihood weighting
$\bimodaly \in \{1, 10, 50\}$
(we keep $\bimodalx = 1$ fixed throughout),
and whether to use PoE or not for $q(z|y)$.
%L1 regularization in $p(y| z)$ in logspace $[5e^{-3}, 5e^{-6}]$,
In addition, each way of training the model has its own
method-specific hyperparameters:
for \jmvae, we choose
$\alpha \in \{0.01, 0.1, 1.0\}$
(the same set of values used in \citep{Suzuki2017});
for \bivcca, we choose
$\mu \in \{0.3, 0.5, 0.7\}$;
for \telbo, we choose
$\unimodaly \in \{1, 50, 100\}$
(we keep $\unimodalx = \bimodalx = 1$).
Thus all methods have the same number of hyperparameters.\footnote{
  %
For \telbo, an additional decision is whether to use the fixed
likelihood
(which only updates $p(y|z)$ in the $\elbo(x,y)$ term)
or not.
We found that turning it off
dropped the \correctness score
from 90.67\% to 85.78\%.
This is because learning the latent space using labels alone will not
result in good alignment to images.
We therefore keep FL turned on throughout the remaining experiments.
} %
We choose hyperparameter values based on performance on the relevant
validation set.
See the supplementary material for more details.



\eat{
In this section, we summarize some of the most important findings
about hyper-parameter choice for the \telbo method.
In the remaining sections, we report results assuming hyperparameters
are set to their optimal value.
}

For \telbo,
we find that it is critical to make $\unimodaly$ sufficiently large;
for example,
if we set $\unimodaly = 1$,
the \correctness score of \telbo on concrete concepts
drops from 90.67\% to 53.43\%. This is consistent with the results
in Section~\ref{sec:results2bit}, which showed the importance of
upweighting the likelihood of the attributes relative to the images.

In terms of the $q(z|y)$ model,
we found that requiring it to be a PoE model (with universal
expert), as opposed to an unrestricted inference network,
slightly reduced performance,
from 90.67\% to 87.34\% (for the \telbo model).
Therefore, in the following experiments,
we only report PoE numbers when  evaluating
abstract concepts.
  
\eat{
In terms of the  frozen likelihood
(which only updates $p(y|z)$ in the $\elbo(x,y)$ term,
and freezes it when optimizing $\elbo(y)$),
we find that turning it off
dropped the \correctness score
from 90.67\% to 85.78\%.
This is because learning the latent space using labels alone will not
result in good alignment to images.
We therefore keep FL turned on throughout the remaining experiments.
}
  
\eat{
Hence
we train three versions of each generative model:
one without PoE on the \iid training set,
one with PoE on the \iid training set,
and one without PoE on the \comp training set.
}

\eat{
We train each model using three objectives:
\telbo, \jmvae and \bivcca.
When using \telbo training,
we use the frozen likelihood modification,
in which we only update $p(y|z)$ in the
aligned $\elbo(x,y)$ term,
and not the unaliged $\elbo(y)$ term) throughout.
This ensures  the latent space is properly shared between images and attributes.
A preliminary experiment in which we turned frozen likelihood off
  dropped the \correctness score of the \telbo model on concrete
  concepts from 90.67\% to 85.78\%.
%  However, it is possible that by suitably changing $\unimodalx$, we
%  could avoid the need to use the fixed likelihood trick. 
}



\input{affine-table}
        
\subsubsection{Evaluating \correctness.}

We start by evaluating the quality of 
models in terms of how correct their samples are.
More precisely, for models trained on the \iid dataset,
we consider 
each of the 240 concrete concepts,
and generate 10 images from each.
For each generated image, we evaluate how many of the
attributes were correctly predicted, and then compute the average
correctness for that concept, and then average over concepts.
%For models trained on the \comp dataset,
%the process is similar, except we just generate 10 images for each of the
%36 concrete concepts in the test set.

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.99\linewidth]{figures/iid_result_figure.pdf}
	\caption{
          Samples  of 2 (previously seen) concrete concepts using 3 different models.
          For each concept, we draw 4 samples from the posterior,
                $z_i \sim q(z|y)$, convert each one to a mean image,
          $\mu_i = E[x|z_i]$, and then show the results.
          The caption at the top of each image (in small font) is the
          predicted attribute values.
         (The observation classifier is fed sampled images, not the
          mean image that we are showing here.)
          The border of the image is black if all attributes are
          correct,  otherwise the border is red.
		}
	\label{fig:correctness}
\end{figure}


The results are shown in Table~\ref{tab:metrics}.
Focusing on the concrete \iid concepts (first block of the table),
we see that \telbo (90.76\%) outperforms \jmvae (86.38\%),
and both methods do significantly better than \bivcca (80.57\%).
To gain more insight,
Figure~\ref{fig:correctness} shows 4 samples
from each of these 3 methods for 2 different concrete concepts,
one chosen at random (bottom row),
and one chosen where the discrepancy in \correctness between \telbo
and \bivcca was maximal.

We see that the images generated by \bivcca are much blurrier than the
other methods,
and are considered  incorrect by the observation classifier.
The blurriness is
because of the $E_{q(z|y)}[\log p(x,y|z)]$ term,
as we discussed above.
For all of our experiments, we use a value of
$\mu=0.7$, which reduces blurriness,
and yields the best \correctness score on the validation set.
Nevertheless, this does not completely eliminate blurriness, as we can see.



From Figure~\ref{fig:correctness} we see that the \jmvae samples look
good.
However, it sometimes makes mistakes
by generating fragments of digit where there should not be any.
This is illustrated in the bottom row, bottom left \jmvae sample,
where there is some ``ghosting'' when generating the digit 1.
This may be because there is no $\KL(q(z|y), p(y))$ term,
which encourages the posterior to be close to the prior,
reducing the chance of the model sampling a $z$ vector far
from the ``familiar'' part of latent space.
\eat{
This may be because the $\alpha$ term,
which weights $\KL(q(z|x,y), q(z|y))$, was too low,
making it more likely for the model to sample a $z$
vector far from the well trained part of latent space.
(However, we did try  a range of $\alpha$ values, and picked the one
that maximized \correctness.)
\kevin{Rama: what value of $\alpha$ did you use for concrete queries?
  Ian thinks your range should have included larger values...}.
}

Table~\ref{tab:metrics}
also shows that the \correctness scores for all methods
are lower on abstract concepts than for concrete concepts.
For example, \telbo drops from 90.76\% to 77.79\% when
we move from conditioning
on 4 attributes to 3.
There are two reasons for this.
First, when evaluating abstract concepts,
we have to use the PoE inference network,
which is somewhat less accurate than models that do not make the PoE assumption. 
%For example, on the concrete concepts,
%the non-PoE version of \telbo  gets 90.76\%,
%whereas the PoE version gets 87.34\%.
Second, abstract concepts are effectively novel concepts that have
never been seen before (since the model is trained only on concrete
concepts).
Indeed, we see that
the \correctness on abstract concepts is comparable to
the \correctness on concrete, but compositionally novel, concepts,
as shown in the last block of the table.
(We discuss the compositional results in more detail below.)



\subsubsection{Evaluating coverage.}

In this section, we evaluate how well each method covers a concept, in
terms of the diversity of the samples it generates.
Note that we only apply this to abstract concepts,
since concrete concepts fully specify all attributes, and hence a
single sample automatically covers the entire concept.

The results are shown in Table~\ref{tab:metrics}.
Once again, we see that \telbo outperforms \jmvae (although the gap is
small), and both methods outperform \bivcca.
To get a better understanding of how well the methods work,
Figure~\ref{fig:coverage} shows some sampled images for concepts at
different levels of abstraction.
In general we see that the samples are correct (consistent with the
attributes that were specified), yet relatively diverse, as desired.
(Note, however, that we manually selected 6 from 10 samples to make
the figure. Automatically generating a diverse set of samples is left
to future work.)

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.99\linewidth]{figures/abstraction.pdf}
	\caption{
		Samples  of 3 abstract concepts using
                the \telbo model. More precisely, for each concept,
                we draw 10 samples from the posterior,
                $z_i \sim q(z|y)$, convert each one to a mean image,
                $\mu_i = E[x|z_i]$, and then manually pick the 6 most diverse ones to show here.
	}
	\label{fig:coverage}
\end{figure}



\subsubsection{Evaluating compositionality.}
\label{sec:evalcomp}

In this section, we evaluate how well methods handle compositionally
novel, concrete concepts.
The results are shown in Table~\ref{tab:metrics}.
We see that the \correctness scores are lower for all methods
than for concrete
concepts in the \iid setting.
This is not surprising, since we are asking the model to extrapolate
rather than interpolate.


\begin{figure}[ht]
	\centering
	\includegraphics[width=0.8\linewidth]{figures/comp_result_figure}
	\caption{
          Samples  of 2 compositionally novel concrete concepts using 3 different models.
          For each concept, we draw 4 samples from the posterior,
                $z_i \sim q(z|y)$, convert each one to a mean image,
          $\mu_i = E[x|z_i]$, and then show the results.
                  The color coding is the same as
                  Figure~\ref{fig:correctness}, namely red border
                  means one or more attributes are incorrect
                  (according to the observation classifier), black
                  border means all attributes are correct.
	}
	\label{fig:compositional}
\end{figure}


As before, we see that \telbo outperforms \jmvae which outperforms
\bivcca. To gain some insight, 
Figure~\ref{fig:compositional} shows some images sampled by the 3
different methods in response to 2 compositionally novel
concrete concepts.
We see that \bivcca seems to have mostly  generated 8's, no matter what the
true concept.
The samples from \jmvae in the top row look reasonable,
but in the bottom row, they are of very poor quality,
with a lot of ghosting;
these artefacts are correctly
detected by
the observation classifier.

\subsubsection{Semantic interpolation with compositionally novel concepts.}

The inference network $q(z|y)$ lets us imagine concepts specified by previously unseen descriptions $y$,
as we discussed in Section~\ref{sec:evalcomp}.
But we can also imagine novel concepts at a
finer level of granularity than obtainable by changing discrete attributes, by moving through the continuous latent space.
Following \citep{White_ICLR_2016}, we perform spherical
interpolation between two ``anchor'' points, $z_1$ and $z_2$.
However, instead of computing these anchors by embedding two
\emph{images}, $x_1$ and $x_2$,
we can compute these anchors by embedding two
\emph{descriptions}, $y_1$ and $y_2$, 
which lets us interpolate between concepts we have never seen before.
More precisely, we sample anchors from the posterior,
$z_1 \sim q(z|y_1)$,
and
$z_2 \sim q(z|y_2)$,
and then perform spherical interpolation to create a path of points
$z_i$. For each point in latent space,
we compute the mean image $\mu_i = E_{p(x|z_i)}[x]$.
We show example results in Figure~\ref{fig:interpolation}.
The model is able to generate plausible hallucinations of novel
concepts purely from symbolic descriptions.


\eat{
Learning good imagination can help us not only conjure
up an image of a concept from a semantic specification, but
also interpolate between such compositionally novel concepts.
This can be useful for a lot of creative explanations, for
instance we can imagine how a woman with a mustache might.
More over we can draw two samples for woman with mustaches
say, with different styles of mustaches and interpolate
between them. We show proof of concept results in the
\mnistaffine world for such behavior. In
Figure~\ref{fig:interpolation}, we show some examples
of compositionally novel concepts and interpolations between
those concepts to demonstrate what the latent space has
learnt between those concepts. We first sample $z \sim q(z| y)$ for a 
novel concept $y$, and
pass the latent sample through $p(x| z)$. We visualize $E[p(x|z)]$
As suggested in~\citet{White_ICLR_2016} we perform spherical interpolation
between two points in latent space as it respects the manifold
structure of the latent space better. We can see that often, only the subset of attriutes which we specify changes for, actually change
 during interpolation with other factors held constant (see third row for example).
}

\begin{figure}[ht]
	\centering
	\caption{
          Results of interpolating in latent space between
          compositionally novel concepts.
          Each row contains two concrete concepts, on the left and right side;
          we then
          spherically interpolating between these
          two concepts in latent space,
          visualize the resulting mean image generated in pixel space.
          These results use the \telbo model trained on the
          \comp dataset using the optimal hyperparameters
          (PoE off, fixed likelihood on,
          $\unimodaly=10$, $\unimodalx=1$,
          $\bimodalx=1$, $\bimodaly=10$,
          $d=10$ latent dimensions).
	}
	\includegraphics[width=\linewidth]{figures/comp_interpolation}
	\label{fig:interpolation}
\end{figure}


%sg_10_multimodal_elbo_comp_pf_False_100_10_10_0_joined_imagination_evalkl_


